Not Just Age but Age and Quality of Information

A versatile scheduling problem to model a three-way tradeoff between delay/age, distortion, and energy is considered. The considered problem called the age and quality of information (AQI) is to select which packets to transmit at each time slot to minimize a linear combination of the distortion cost, the age/delay cost and the energy transmission cost in an online fashion. AQI generalizes multiple important problems such as age of information (AoI), the remote estimation problem with sampling constraint, the classical speed scaling problem among others. The worst case input model is considered, where the performance metric is the competitive ratio. A greedy algorithm is proposed that is shown to be 2-competitive, independent of all parameters of the problem. For the special case of AQI problem, a greedy online maximum weight matching based algorithm is also shown to be 2-competitive.

==> NewProof-Nived.tex <==
We have that $\sum_t v_A(S_t,t) = ALG$ where $S_t = \{1,\dots,A_t\}$. We also have that $\sum_t v_{\opt}(S_t^*,t) = \opt$ where $S_t^* = \{1,\dots,O_t\}$.

Claim: ALG does not serve a packet before OPT. This can be proved by contradiction at any time. Assume that ALG decides to serve packets $S_t = \{p_1,p_2,\dots,p_t\}$ at time $T$. These are part of the locally best solution at that time. Let OPT decide to serve $S_t^* = \{p_1^*,p_2^*,\dots,p_t^*\}$ and define $S^\cap_t = S_t \cap S_t^*$ and $S_t^+ = S_t \setminus S_t^*$ and $S_t^- = S_t^* \setminus S_t$.
We claim that $S_t^+ = \phi$. To show this, we first assume that $|S_t^+|=1 = |\{p_1\}|$ and show a contradiction. Then,
\begin{enumerate}
\item The best local matching between waiting resources at time $t$ with slots is $M_t$. $M_t \setminus \{(p_1,t)\}$ gives the most improvement when $(p_1,t)$ is added to it. We split the analysis into $2$ cases:
\begin{description}
\item[$|S_t^-| \ge 1$] WLOG assume that $p_1^* \in S_t^-$. Let the packet $p_1^*$ be scheduled at some time $t_1 \ne t$ in $M_t$ ($p_1^*$ cannot be scheduled at time $t$ by definition of $S_t^-$ which it is a member of). Swapping $p_1^*$ and $p_1$ in OPT cannot give a better solution (by definition of OPT). Swapping $p_1^*$ and $p_1$ in $M_1t$ gives a worse local solution. The only cost that needs to be compared is the delay cost as in the process of 
\end{description}
\end{enumerate}

==> NewProof.tex <==
Notation: Let at slot $t$, let $A_t$ and $O_t$ be the number of energy slots used by the matching algorithm and the $\opt$. Let $v_{*}(S, t)$ be the value accrued by the $*$ algorithm when set of energy slots $S$ is used at time slot $t$. 

For the special case when the packet $p$'s value if matched to the $k^{th}$ energy slot of time slot $t$ is $v_p - (t-A_p) - g'(k)$, where $A_p$ is the arrival time of packet $p$, and $g'(k) = g(k)-g(k-1)$.

\noindent Claim 1:  For $S = \{1, \dots, A_t\},\ v_{A}(S, t) \ge v_{\opt}(S, t)$.
\begin{proof}
We can assume this, because of the reason that at any time $t$, the action of swapping the slots of two packets in the locally optimal solution $L$ generated by the matching algorithm does not change the total value of $L$. All the discarded packets discarded at a particular time must also have the least valuation (excluding energy cost) at that time. We can therefore assume that the locally optimal solution generated by the matching algorithm is reordered such that packets are transmitted in decreasing value (through slots and time) and the $\mathcal{P}_{A}(t) - \sum_{t' > t} A_{t'}$ packets with least value are discarded. This means that the set of packets transmitted by the matching algorithm at time $t$ is the set of highest value packets (of size $A_t$) among all outstanding packets at time $t$. Lemma \ref{lem:007} states that the set of outstanding packets for the matching algorithm will always be a superset of outstanding packets in the $\opt$ schedule at time $t$. Therefore, $\opt$ cannot transmit a set of packets (of size $A_t$) at time $t$ of more value than sent by the matching algorithm (in the first $A_t$ slots) at time $t$.
\end{proof}

\noindent Claim 2:  For $S_1 = \{1, \dots, O_{t}-A_{t}\}$, and $S_2 =  \{A_{t}+1, \dots, O_{t}-A_{t}\}$,
$$v_{A}(S_1, t+1) \ge v_{\opt}(S_2, t).$$
\begin{proof}
If this was not the case, then the locally optimal solution could be improved by scheduling at time $t$ (in slots $A_{t+1}$ to $O_t$) those packets  scheduled by $\opt$ in slots $\{A_{t+1}, \dots, O_t \}$ and discarding all those packets scheduled by the matching algorithm in slots $1,\dots,O_t -A_t$ at time $t+1$.
\end{proof}

\begin{theorem}
Matching algorithm is $2$-competitive.
\end{theorem}
\begin{proof}
At any time $t : O_t > A_t$, define $S_A^t = \{1,2,\dots,A_t\}$ and $S_{\opt}^t = \{1,2,\dots,O_t\}$:
\begin{align}
v_{\opt} (S_{\opt}^t ,t) &\overset{(i)}{\le} v_{\opt} (S_A^t, t) + v_{\opt} (S_{\opt}^t \setminus S_A^t, t) \nonumber\\
&\overset{(ii)}{\le} v_{A} (S_A^t, t) + v_{A} (\{1,\dots,O_t-A_t\},t+1) \nonumber\\ &\le v_{A} (S_A^t, t) + v_{A} (S_A^{t+1},t+1) \label{eq:A>O}
\end{align}
where $(i)$ relies on $A_t \le O_t$, $(ii)$ follows from Claim 1 and 2. On the other hand, a any time $t : O_t \le A_t$, 
\begin{align}
v_{\opt} (S_{\opt}^t ,t) &\overset{(i)}{\le} v_{\opt} (S_A^t, t) \nonumber\\
&\overset{(ii)}{\le} v_{A} (S_A^t, t)  \label{eq:A<=O}
\end{align}
where $(i)$ relies on $A_t \le O_t$, $(ii)$ follows from Claim 1.
\end{proof}
Summing (\ref{eq:A>O}) and (\ref{eq:A<=O}) over $t : O_t > A_t $ and $t : O_t \le A_t$ respectively, and noting that $C_{A} =  \sum_t v_{A} (S_A^{t},t) $ and $C_{\opt} = \sum_t v_{\opt} (S_{\opt}^{t},t)$ the Theorem follows.

\begin{lemma}\label{lem:ordertime} If two packets $p_1$ and $p_2$ arrive at time $t_1$ and $t_2$, where 
$t_2>t_1$ and if both are transmitted by the matching algorithm/$\opt$, then $p_1$ is never transmitted in a slot later than $p_2$.
\end{lemma}
\begin{proof} Proof is immediate, since otherwise we can swap the two packets and increase the valuation.
\end{proof}
\begin{lemma}\label{lem:ordervalue} If two packets $p_1$ and $p_2$ with value $v_1\le v_2$ arrive in the same time slot and both are transmitted by any algorithm, then without loss of generality we can assume that $p_1$ is not transmitted later than $p_2$. 
\end{lemma}
\begin{proof} Since otherwise, we can swap the two packets without changing the overall valuation.
\end{proof}

\begin{lemma}\label{lem:domination} With input $\sigma$, if any packet $p$ is transmitted by $\opt$ in time slot $t$. Then packet $p$ is never transmitted by $\opt$ in a time slot later than $t$ if the input is $\sigma \cup \{q\}$ where $q$ arrives after time $t$, i.e., augmented by a packet that arrives after time slot $t$.
\end{lemma}

Let the time slot at which packet $p$ is sent by the $*$ algorithm be $T_{*}(p)$.
\begin{lemma} \label{lem:007}For every packet $p$ transmitted by both $\opt$ and the matching algorithm, $T_{\opt}(p) \le T_{A}(p)$. Every packet discarded by $\opt$ is also discarded by the matching-algorithm.
\end{lemma}
\begin{proof}

[Contradiction] Assume that the claim is not true. Then consider the earliest time slot $t$, for which there exists a packet $p$ such that $T_{A}(p) = t$ while  $T_{\opt}(p) > t$ or $p$ is discarded.
Then until time slot $t-1$ all packets sent by algorithm have also been sent by the $\opt$ by time slot $t-1$. Thus, the set of available packets at time slot $t$ with the algorithm 
$\cP_A(t) = \{p_1, \dots p_k\}$ (indexed in increasing order of their increasing arrival time slots, and in increasing order of value if arrived at the same time slot)  contains the set of available packets at time slot $t$ with the $\opt$
$\cP_\opt(t)$, i.e., $\cP_\opt(t) \subseteq \cP_A(t)$. Consider the earliest packet $p_i$ among the packets of $\cP_A(t)$ that the $\opt$ does not transmit at time $t$, while the algorithm does.

From Lemma \ref{lem:ordertime} and Lemma \ref{lem:ordervalue}, we know that the algorithm also transmits packets $p_1 \dots p_{i-1}$ packets in time slot $t$ together with $p_i$. From Lemma \ref{lem:ordertime} and Lemma \ref{lem:ordervalue}, we also know that the $\{p_k, k\ge i\}  \in \cP_\opt(t)$.
 Moreover, by the definition of $p_i$, $\opt$ transmits all packets among $\{p_1 \dots p_{i-1}\} \cap \cP_\opt(t)$. Moreover, since $\opt$ is not transmitting $p_i$ it will not transmit any packets from $\{p_k, k\ge i\}$ of $\cP_\opt(t)$ because of Lemma \ref{lem:ordertime} and Lemma \ref{lem:ordervalue}.

Let no new packets arrive after time slot $t$. Then the $\opt$'s transmission schedule for packets $\{p_k, k\ge i\}$ of $\cP_\opt(t)$ after time slot $t$ can also be used by the matching algorithm for packets $\{p_k, k\ge i\}$ that it has, which is a candidate for packets $\{p_k, k\ge i\}$ among all schedules chosen by the matching algorithm's schedule, but rejected by it. Thus, we get a contradiction to the optimality of $\opt$.

Following Lemma \ref{lem:domination}, the same conclusion holds even when more packets arrive after time slot $t$.

\end{proof}

\noindent We define the value of subpackets sent at time $t$ in the set of slots $S$ by algorithm $*$ as $v_{*} (S,t)$. Then,

\noindent Claim 1: $A_t$ is a decreasing function of $t$ in the local solution generated by the matching algorithm.

\noindent Claim 2: For $S = \{1,\dots,A_t\}$, $v_{A} (S,t) \ge v_{\opt} (S,t)$.
\begin{proof}
Consider the locally optimal solution $L$ generated by the matching algorithm at any time $t$. Assume that for each packet $p \in \mathcal{P}_A (t)$, $A_p$ sub-packets are scheduled in $L$. Order the packets in $\mathcal{P}_A (t)$ in increasing order of $A_p$ as $(p_{i_1}, p_{i_2}, \dots)$.  Since the delay accumulated by a packet in $L$ is governed by the last time at which a subpacket is transmitted, subpackets in $L$ can be rearranged (within the same set of slots $\{ \forall i,\ t_i \to A_{t_i}\}$) such that all transmitted subpackets of $p_{i_1}$ are all scheduled first followed by those of $p_{i_2}$ and so on, which minimizes the total delay. The set of transmitted subpackets for each packet are the first $A_p$ subpackets when ordered in decreasing order of valuation. Conclusion: {\color{red} [the order in which subpackets are scheduled in the local matching is: all the subpackets of packet $p_{j_1}$, then all subpackets of $p_{j_2}$ and so on where $\{ p_{j_i} \}$ is ordered in increasing order of the number of of subpackets of that packet that the local matching schedules]} This does not translate to $v_{A} (S,t) \ge v_{\opt} (S,t)$ because in the no-subpacket case, the matching algorithm schedules the maximum value packets first (among the waiting packets) which the $\opt$ cannot dominate. But here the matching algorithm does not transmit the maximum value packets first (in fact it might even transmit the least value packets first).
\end{proof}

\begin{lemma}\label{lem:ordertimesubpacks}
Let for packet $k$, consider the set of outstanding sub-packets $\cS_k$ at time slot $t$ that will eventually be transmitted by algorithm $*$. 
Let the sub-packets of $\cup_k \cS_k$ be ordered in increasing order of $|\cS_k|$, i.e., $\cS_{k_1},   \cS_{k_2}, \dots $ where $|\cS_{k_1}| \le |\cS_{k_2}|, \dots, $.  If $|\cS_{k_i}| = |\cS_{k_j}|$ then we order them in increasing order of their  time of arrival.
Then the matching algorithm or the $\opt$, transmits the sub-packets in order as described above.
\end{lemma}
\begin{proof} Consider a fixed time slot $t$. If $|\cS_{k_i}| = |\cS_{k_j}|$, then the claim that the sub-packets be transmitted in order of their increasing order of arrival is immediate from Lemma \ref{lem:ordertime}.
For the case when $|\cS_{k_i}| \le |\cS_{k_j}|$, let $d_i$ and $d_j$ be the delay accumulated by packet $k_i$ and $k_j$ until time slot $t-1$. If packet $p_*$ arrives at time slot $t$, $d_*=0$. Then if any subpacket of $\cS_{k_j}$ is transmitted before any subpacket of $\cS_{k_i}$, we can swap the two subpacket's location of transmission without changing the sum of the incremental accumulated delay of packet $k_i$ and $k_j$ starting from $d_i$ and $d_j$.
\end{proof}

%\begin{lemma}\label{lem:ordertimesubpacks} Consider two packets $p_1$ and $p_2$ that arrive at time $t_1$ and $t_2$, where 
%$t_2>t_1$. If the sub-packet $p_j^i$ of packet $i$ is transmitted at time $t_j^i$ by the matching algorithm or the $\opt$. Then 
%$t_j^1 \le t_j^2$ for any $j$.
%\end{lemma}
%\begin{proof} Proof is immediate, since otherwise we can swap the two packets and increase the valuation.
%\end{proof}
Consider the set of packets for which both the algorithm and the $\opt$ transmit the same number of subpackets. For example, for the case when an algorithm is valid only if it transmits all subpackets.
Let the time slot at which subpacket $p_k^j$ of packet $j$ is sent by the $*$ algorithm be $T_{*}(k,j)$.
\begin{lemma} $T_{\opt}(k,j) \le T_{A}(k,j)$.
\end{lemma}
\begin{proof} 

[Contradiction] Assume that the claim is not true. 
Consider the earliest time slot $t$ where some subpacket $j$ of packet $k$ ($p_j^k$) that is transmitted by the matching algorithm before the $\opt$. Index the subpackets of $\cP$ and $\cP_{\opt}$ in the order described in Lemma \ref{lem:ordertimesubpacks}. 
%Let $t$ be the slot when the algorithm transmits $p_j^k$. 
Let $\cP$ and $\cP_{\opt}$ be the set of outstanding subpackets with the algorithm and the $\opt$ at slot $t$. By the contradiction hypothesis' choice of $t$, $\cP_{\opt}\subseteq \cP$.


%As before, index the sub-packets in $\cP$ in increasing order of arrival and increasing order of value for packets arriving in the same slot.
%From Lemma \ref{lem:ordertimesubpacks}, we know that the set of outstanding packets with the algorithm include all sub-packets $p_k^i$ for all packets $i$ that have arrived after packet $j$. 

Define $\mathsf{major} = \{\cS_\ell : |\cS_\ell| \ge |\cS_{k}|\} $. Clearly, $\mathsf{major} \subseteq \cP$.
We also have that $\mathsf{major} \subseteq \cP_{\opt}$, since $\opt$ is not transmitting $p_k^j$ in slot $t$. 

Since the algorithm is transmitting $p_j^k$ it will also transmit all the packets of $\cP$ that lie before it in the indexed order, call them $\mathsf{minor}$.  Moreover, by the definition of $p_j^k$, $\opt$ transmits all packets among $\mathsf{minor} \cap \cP_\opt(t)$.

Let no new packets arrive after time slot $t$. Then the $\opt$'s transmission schedule for packets of $\mathsf{major} \subseteq \cP_\opt(t)$ after time slot $t$ can also be used by the matching algorithm for packets of set $\mathsf{major}$ that it has, which is a candidate for packets $\mathsf{major}$ among all schedules chosen by the matching algorithm's schedule, but rejected by it. Thus, we get a contradiction to the optimality of $\opt$.

Following Lemma \ref{lem:domination}, the same conclusion holds even when more packets arrive after time slot $t$.
\end{proof}

[It would be nice to prove the following Lemma but does NOT appear to be true.]
\begin{lemma} The number of subpackets for any packet $k$ transmitted by the $\opt$ is at least as much as transmitted by the matching algorithm.
\end{lemma}

==> ProofLemma1.tex <==
For proving Lemma \ref{lemma:rho-inc}, we assume that at every time instant, either a vertex in $B$ locks or a new vertex from $A$ arrives. In the context of binary AQI problem, that is 
sufficient, since the packets (nodes $a$) arrive only at the beginning of the slot, 
while time slots (node $b_{t,i}$'s) expire at the end of time slot.

\begin{proof}[Lemma 1]
\begin{definition}[flow network] \label{def:flow-network}
A flow network is a directed graph $G = (V,E)$ with distinguished vertices denoted $s$ (source) and $t$ (sink). Every edge $e \in E$ is associated with a weight $w_e$ and a capacity $c_e$, and is referred to as a \textit{$w_e$-weight $c_e$-capacity edge}.
\end{definition}

\begin{definition}[flow] \label{def:flow}
Given a flow network $G=(V,E)$, with weights $w_e$ and capacity $c_e$ on every edge $e \in E$, a flow $f = \{f_e : e \in E\}$ is a set satisfying the following properties:
\begin{enumerate}
\item $\forall e \in E,\ 0 \le f_e \le c_e$. The flow on an edge is positive and cannot exceed the capacity of that edge. If the flow through edge $e$ is equal to $c_e$, it is said to be saturated.
\item For an edge $e = (u,v) \in E$, we use $t(e)$ to denote $u$ and $h(e)$ to denote $v$. Then, 
\begin{equation*}
\forall v \in V \setminus \{s,t\},\ \sum_{e \in E : t(e) = v} f_e = \sum_{e \in E : h(e) = v} f_e
\end{equation*}
Given a flow $f$, $f_e$ is referred to as the flow through edge $e$. The quantity $\sum_{e \in E} f_e.w_e$ is referred to as the weight of the flow.
\end{enumerate}
\end{definition}


    For any vertex $b$, in case $t > T_b$, the proof is trivial, since $\rho_t(b)$ is defined as $\nu_b$ for any locked vertex and remains fixed throughout.
    For $t \le T_b$, the proof follows separately for 3 cases, where either
    \begin{description}
    \item[Vertex $b' \ne b$ is locked ($t < T_b$):] Since there is no arrival, $A_t = A_{t-1}$. The set of locked edges at time $t$, $L_t = L_{t-1} \cup e'$, where $e'$ is the edge in $L_{t}$ incident on $b'$ in the matching $M(A_{t-1},B,F_{t-1})$.
    By definition, since edge $e'$ is incident on $b'$ in the matching $M(A_{t-1},B,L_{t-1})$, it is the edge that is locked in at time $t$. The two matchings $M(A_{t-1},B,L_t)$ and $M(A_{t-1},B,L_{t-1})$ are identical. The only difference is that the edge $e'$ is a part of $L_t$ in $M(A_{t-1},B,L_t)$ since $b'$ locks at time $t$, but in $M(A_{t-1},B,L_{t-1})$ $e'$ is not included among the edges in $L_{t-1}$ since $b'$ has not locked yet. Therefore,
    \begin{equation} \label{eq:001} W(A_{t-1},B,L_t) = W(A_{t-1},B,L_{t-1})
    \end{equation}
    The matching $M(A_{t-1},B \setminus \{b\}, L_{t-1})$ is the optimal matching between $A_{t-1}$ and $B \setminus \{b\}$ when constrained to include $L_{t-1}$. Therefore, it cannot have lower weight than any matching between $A_{t-1}$ and $B \setminus \{b\}$ when constrained to include $L_t = L_{t-1} \cup \{e'\}$ - one such matching being $M(A_{t-1},B \setminus \{b\}, L_{t})$.
    \begin{equation} \label{eq:002}
        W(A_{t-1},B \setminus \{b\},L_t) \le W(A_{t-1},B \setminus \{b\}, L_{t-1})
    \end{equation}

Subtracting (\ref{eq:002}) from (\ref{eq:001}) and using the fact that $A_t = A_{t-1}$, from the definition of $\rho_t(b)$ the Lemma follows for this case.
    \item[Vertex $b$ is locked ($t = T_b$):] Since $t=T_b$, the weight of the edge $e=(a',b)$ to $b$ in $M(A_{t-1},B, L_{t-1})$, $w_{a'b}$ is equal to $\nu_b$ (as this edge is locked at time $T_b$). A valid matching from the vertices in $A_{t-1}$ to $B \setminus \{b\}$ that includes $L_{t-1}$ is: $ M(A_{t-1}, B \setminus \{b\}, L_{t-1})$ with the edge $e$ removed and with $a'$ discarded. This matching has weight $W(A_{t-1},B,L_{t-1}) - w_{a'b} = W(A_{t-1},B,L_{t-1}) - \nu_b$. Since $M(A_{t-1}, B \setminus \{b\}, L_{t-1})$ is the optimal matching from $A_{t-1}$ to $B\setminus \{b\}$ that includes $L_{t-1}$, we have that:
    \begin{align*}
        &W(A_{t-1}, B \setminus \{b\}, L_{t-1}) \ge W(A_{t-1},B,L_{t-1}) - \nu_b \\
        \Rightarrow \ &\nu_b \ge W(A_{t-1},B,L_{t-1}) - W(A_{t-1}, B \setminus \{b\}, L_{t-1}) = \rho_{t-1}(b) \\
        \Rightarrow \ &\rho_t{b} \ge \rho_{t-1}(b)
    \end{align*}
    \item[Vertex $a \in A$ arrives:] We begin with a brief proof outline. In order to prove the Lemma statement in this case, we construct a flow network $N_{12}$ and consider a flow $f_{12}$ on it with weight $W(A_t,B \setminus \{b\},L_t) + W(A_{t-1},B,L_{t-1})$. We then consider $f^*$, the maximum-weight flow over $N_{12}$ and show that it can be decomposed into valid flows, $F_1$ and $F_2$ such that the weight of $F_1$ is upper bounded by $W(A_t,B,L_t)$ and the weight of $F_2$ by $W(A_{t-1},B \setminus \{b\},L_{t-1})$. Using $H(f)$ to denote the weight of a flow $f$ over the network $N_{12}$, we have:
\begin{align*}
W(A_{t},B \setminus \{b\},L_t) + W(A_{t-1},B,L_{t-1}) &= H(f_{12}) \\
&\overset{(i)}{\le} H(f^*) \\
&= H(F_1) +H(F_2) \\
&\le W(A_{t},B,L_t) + W(A_{t-1},B \setminus \{b\},L_{t-1}) \\
\Rightarrow W(A_{t-1},B,L_{t-1}) - W(A_{t-1},B \setminus \{b\},L_{t-1}) &\le W(A_{t},B,L_t) - W(A_{t},B \setminus \{b\},L_t) \\
\Rightarrow \rho_{t-1}(b) &\le \rho_t(b)
\end{align*}
where $(i)$ follows by optimality of $f^*$.

In order to generate $N_{12}$, we first construct two flow networks $N_1$ and $N_2$. $N_{12}$ is then generated by appropriately superimposing $N_1$ and $N_2$. Since no vertex locks at time $t$, $L_t = L_{t-1}$ (no new edges are locked). We also have that $A_t = A_{t-1} \cup \{a\}$. As shown in Figure \ref{fig:1c}, we build a flow network $N_1$ on the bipartite graph with vertices $A_t \cup B \setminus \{b\}$ and will consider a flow $f_1^*$ on it having weight $W(A_t,B \setminus \{b\},L_t)$ on it. $N_1$ is generated by first adding source $s_1$ and sink $t_1$, where $s_1$ is adjacent to every vertex in $A_t$ via $0$-weight $1$-capacity edges and $t_1$ is adjacent to every vertex in $B \setminus \{b\}$ through $0$-weight $1$-capacity edges. $B \setminus \{b\}$ is also augmented with $|A_t|$ dummy vertices, one for each vertex in $A_t$. Each vertex $a \in A_t$, is connected to its corresponding dummy vertex $d_a$ through a $0$-weight $1$-capacity edge. Each dummy vertex is also connected to $t_1$ through a $0$-weight $1$-capacity edge. $N_1$ now has $|A_t|$ left nodes and $|B|-1+ |A_t|$ right nodes. The flow $f_1^*$ is defined as the max-weight flow over $N_1$ under the constraint that every edge in $L_{t-1}$ must be saturated with unit flow. The presence of dummy nodes ensures that every vertex in $A_t$ is saturated with $1$ unit of flow, without affecting the value of the flow, which is $W(A_t,B \setminus \{b\},L_{t-1})$.
    
A similar procedure is followed to generate a flow network $N_2$ on the bipartite graph with vertices $A_{t-1} \cup B$. $N_2$ has $|A_{t-1}|$ left nodes and $|B|+|A_{t-1}|$ right nodes. We consider the max-weight flow over $N_2$ under the constraint that every edge in $L_{t-1}$ is saturated with unit flow and denote this as $f_2^*$. A similar argument as in the case of $f_1^*$ concludes that $f_2^*$ has weight equal to $W(A_{t-1},B,L_{t-1})$.

Flow-networks $N_1$ and $N_2$ are defined over a common set of vertices with the exception of $b$ (not in in $N_1$),  $a$ and $d_a$ (not in $N_2$) where $d_a$ is the dummy vertex corresponding to $a$. $N_1$ and $N_2$ are then superimposed to generate the network $N_{12}$ - each vertex is merged with its counterpart, and for edges between two such vertices, the capacity is doubled, but the weight is kept unchanged. The weights and capacities of edges that are incident on either $a, d_a$ or $b$ are kept unchanged. As shown in Figure \ref{fig:2a}, the vertex set of $N_{12}$ is $A_t \cup B \cup D \cup \{s_1,t_1\}$, where $D$ is the set of dummy nodes for $A_t$.

    Since $f_1^*$ is a valid flow on $N_1$ and $f_2^*$ is a valid flow on $N_2$, the superposition of $f_1^*$ and $f_2^*$ denoted $f_{12}$ having weight $W(A_t,B\setminus\{b\},L_t) + W(A_{t-1},B,L_t)$ is a valid flow on $N_{12}$. Furthermore, $f_{12}$ is constrained to have exactly $2$ units of flow through every edge in $L_t$ (since in both $f_1^*$ and $f_2^*$, every edge in $L_t$ has unit flow). Defining $f^*$ as the max-weight flow over $N_{12}$ with the constraint that every edge in $L_t$ has a flow of $2$, and recalling that $H(f)$ denotes the weight of flow $f$ over the network $N_{12}$, it follows that:
    \begin{align}
    H(f^*) &\ge W(A_t,B \setminus \{b\},L_t) + W(A_{t-1},B,L_t) \nonumber \\
    &\overset{(i)}{=} W(A_t,B \setminus \{b\},L_t) + W(A_{t-1},B,L_{t-1}) \label{eq:003}
    \end{align}
    where $(i)$ follows from the fact that no node is locked in at time $t$ and hence $L_t = L_{t-1}$. Due to the presence of dummy nodes having $0$-weight edges, there are multiple candidates for $f^*$ having the same total weight. One such candidate is the maximum weight flow on $N_{12}$ excluding the dummy vertices (every vertex except $a$ has a flow of $0$ or $2$, and $a$ has a flow of $0$ or $1$ through it). Henceforth, the maximum-weight flow described below is referred to as $f^*$: \begin{enumerate}
        \item the flow of every unsaturated (having flow $0$) vertex in $A_t \setminus \{a\}$ is saturated by passing $2$ units of flow through the $0$-weight edge to its dummy node.
        \item If $a \in A_t$ is unsaturated, unit flow is pushed through the $0$-weight $1$-capacity edge to its dummy node $d_a$.
    \end{enumerate}
    Every vertex in $A_t$ has $2$ units of flow through it in $f^*$, except for $a$, which has unit flow through it.

    In the following, we decompose the edges in $f^*$ into $2$ sets $F_1$ and $F_2$, and show that the $F_1$ corresponds to a valid matching between $A_t$ and $B$ with the condition that all edges in $L_t$ must be included, while $F_2$ corresponds to a valid matching between $A_{t-1}$ and $B \setminus \{b\}$ under the same condition that the edges in $L_t$ are included in the matching. The decomposition is as follows:
    \begin{enumerate}
    \item by definition of $f^*$, every edge to $A_t$ from $s_1$ is saturated. Therefore, edges to $A_t \setminus \{a\}$ are split into two each having unit capacity, unit flow and weight unchanged as before, and given to $F_1$ and $F_2$. In Figure \ref{fig:3}, these correspond to the edges $(s_1,a_1),(s_1,a_2),(s_1,a_3)$ and $(s_1,a_4)$. The edge $(s_1,a)$ is also given to $F_1$.
    \item Consider those edges in $f^*$ between $A_t$ and $B \cup D$ (all such edges have capacity at-most $2$) that are saturated with $2$ units of flow. In Figure \ref{fig:3}, these correspond to the edges $(a_1,b_2)$ and $(a_2,b_1)$. Every edge in $L_t$ satisfies this criterion. Each such edge is divided into two identical $1$-capacity edges with unchanged weight and unit flow through them, and one is added to $F_1$ while the other is added to $F_2$. These edges are then removed from $f^*$. The rest of the edges between $A_t$ and $B \cup D$ in $f^*$ must have unit flow through them.
    %\item[2] Starting from vertex $a$, form a path alternating between vertices in $A_t$ and in $B$ through the remaining edges with unit flow in $f^*$. Odd edges are added to $F_1$, and even edges are added to $F_2$. These edges are then removed from $f^*$.
    %\item[3] If vertex $b$ is not covered in the previous step, then a path is traced through edges with unit flow starting from $b$ and alternating between $B$ and $A_t$ through edges with unit flow in $f^*$. Note that such a path cannot involve edges removed in Step 2 even if they were not removed, because it would mean that the path in Step 2 can be traced back to connect $b$ with $a$ - a contradiction, since we assume $b$ is not covered in the previous step. In this path, odd edges are added to $F_2$, and even edges are added to $F_1$. These edges are then removed from $f^*$.
    \item At the end of Step 1, every remaining edge in $f^*$ between $A_t$ and $B \cup D$ has unit flow through it. Starting from any vertex in $A_t \cup B \cup D$ on which is incident a \textbf{single} edge with unit flow through it ($a$ and $b$ are valid such starting points), form a path alternating between vertices in $A_t$ and $B \cup D$ using the edges remaining after Step 1 in $f^*$. Edges in this path are placed alternately into $F_1$ and $F_2$ in such a way that the edge involving $a, b$ or $d_a$ (dummy node corresponding to $a$) is put into $F_1$. Referring back to Figure \ref{fig:3}, starting from $a$, we follow the path ${\color{olive} (a,b_3)} \to {\color{teal}(b_3,a_3)} \to {\color{olive}(a_3,b_4)} \to {\color{teal}(b_4,a_4)} \to {\color{olive}(a_4,b)}$ and add odd edges to $F_1$ and even edges to $F_2$. It is always possible for edges involving $a$, $b$ or $d_a$ be put into $F_1$, since any path starting in $A_t$ and ending in $B \cup D$ or vice-versa would have to be of odd parity (if $(a,v_1)$ is placed in $F_1$ for some $v_1$, then $(v_2,b)$ for some $v_2$ would have to be placed in $F_1$ without exception). On the other hand, if a unit-flow edge is incident on $d_a$:
    \begin{enumerate}
        \item it must be connected to $a$ (by definition of dummy edge).
        \item only one such unit-flow edge exists (since no edge can exist from $d_a$ to any other vertex).
    \end{enumerate}
    Hence if $a$ is placed in $F_1$ and a unit flow edge to $d_a$ exists, the path must have a single edge $(a,d_a)$. The set of edges along this path is removed from $f^*$. Step 2 is repeated until no vertex remains in $A_t \cup B \cup D$ onto which a single unit-flow edge in $f^*$ is incident.
    \item Since no vertex in $A_t \cup B \cup D$ with a single unit-flow edge incident on it in $f^*$ remains, the remaining unit-flow edges in $f^*$ must form cycles that alternate between $A_t$ and $B \cup D$. Moreover, such cycles are guaranteed to be simple - for every every vertex $a' \in A_t$ the incoming flow along the edge to $s_1$ cannot exceed $2$ units and hence $a'$ can only have at-most $2$ unit-flow edges incident on it. Similarly, for every vertex $b' \in B \cup D$ the outgoing flow along the edge to $t_1$ cannot exceed $2$ units, implying that it can cannot have more than $2$ unit-flow edges incident on it. Such cycles are also guaranteed to have an even number of edges which follows by a simple parity argument. Each edge in such a cycle is alternately assigned to $F_1$ and $F_2$ with arbitrary assignment to the starting vertex.
    \item The final set of remaining edges $E_{t_1}$ are those from $B \cup D$ to $t_1$. Every edge having $2$ units of flow through it in $f^*$ is split into unit capacity edges having unchanged weight and unit-flow through them. A subset $E_1$ of these edges is chosen such that for $F_1$, the flow input into every vertex in $B \cup D$ is matched by the flow output due to the corresponding edge in $E_1$. The set $E_1$ is added to $F_1$. The remaining edges $E_{t_1} \setminus E_1$ match the flow input for every vertex in $B \cup D$ in $F_2$. This is because $f^*$ is a valid flow, and hence the flow input at every vertex in $B \cup D$ due to $F_1 \cup F_2$, is exactly matched by the corresponding edge in $E_{t_1}$.
    \end{enumerate}

	\input{image.tex}    
    
    By this construction, the set $F_1$ represents a valid flow over a network with source $s_1$, sink $t_1$, left nodes $A_t$ and right nodes $B \cup D$ and every edge in $L_t$ has unit flow through it. On the other hand $F_2$ represents a valid flow over a network with source $s_1$, sink $t_1$, left nodes $A_{t} \setminus \{a\}$ and right nodes $(B \setminus \{b\}) \cup (D \setminus \{d_a\})$ and once again, every edge in $L_t$ has unit flow through it. Thus, the sum of weights of these two flows, which is equal to $H(f^*)$ must be upper bounded by the maximum flows over the respective networks (conditioned on the fact that edges in $L_t$ must all have unit flow through them). Thus,
    \begin{align}
        H(f^*) &\le W(A_t, B, L_t) + W(A_t \setminus \{a\}, B \setminus \{b\}, L_t) \nonumber \\
        &\overset{(i)}{=} W(A_t, B, L_t) + W(A_{t-1}, B \setminus \{b\}, L_{t-1}) \label{eq:004}
    \end{align}
    where $(i)$ follows from the fact that $a$ is the node that arrives at time $t$, and also from the fact that no node is locked in at time $t$ and hence $L_t = L_{t-1}$. Thus from (\ref{eq:003}) and (\ref{eq:004}), it follows that
    \begin{equation*}
        \rho_{t-1}(b) \le \rho_t(b)
    \end{equation*}
    \end{description}

\end{proof}
